Learning to Learn Graph Topologies

Learning a graph topology to reveal the underlying relationship between data entities plays an important role in various machine learning and data analysis tasks. Under the assumption that structured data vary smoothly over a graph, the problem can be formulated as a regularised convex optimisation over a positive semidefinite cone and solved by iterative algorithms. Classic methods require an explicit convex function to reflect generic topological priors, e.g. the $\ell_1$ penalty for enforcing sparsity, which limits the flexibility and expressiveness in learning rich topological structures. We propose to learn a mapping from node data to the graph structure based on the idea of learning to optimise (L2O). Specifically, our model first unrolls an iterative primal-dual splitting algorithm into a neural network. The key structural proximal projection is replaced with a variational autoencoder that refines the estimated graph with enhanced topological properties. The model is trained in an end-to-end fashion with pairs of node data and graph samples. Experiments on both synthetic and real-world data demonstrate that our model is more efficient than classic iterative algorithms in learning a graph with specific topological properties.

==> bins.tex <==


%{\HC 
to augment the topological difference between $G_
X$ from unrolling module and the target graph $G_Y \in \mathcal{G}$.  Different from \cite{jin2020-graph2graph}, the mapping is not multimodal in our case as the unrolling module returns permutation-invariant estimation.

\Note{SC: overall intuition is missing.} 
% Methods ===========
\begin{comment}
{\HC The pseudo-code of these algorithms are often written in a few lines of handcrafted rule to iteratively update until the graph estimation converges.} For example, G-ISTA \cite{guillot2012iterative} applies proximal gradient descent to estimate $\*K$ in $l_1$ regularised log-likelihood maximisation, which iteratively update 
\begin{equation}
    \*K^{(t+1)} \leftarrow \text{prox}_{\gamma^{(t)}, ||\cdot||_1} \Big( \*K^{(t)} - \gamma^{(t)} (\*X\*X^{\top} - \*K^{(t)-1}) \Big)
\end{equation}%
where the proximal operator $\text{prox}_{\gamma^{(t)}, {||\cdot||_1}}(\cdot)$ is an entrywise soft-threshold operator on gradient-updated matrix with a step size $\gamma^{(t)}$. 
Note that G-ISTA and many other classical iterative algorithms \cite{Banerjee2008ModelData, DAspremont2008} simply solve $l_1$ regularised maximum log-likelihood estimation of $\*K$ and {\HC do not draw a further connection to the graph Laplacian $\*L$.   It can be achieved by adding one more constraint such that off-diagonal entries are non-positive, which however complicates the design of the update rule.} \par  
\end{comment}




\begin{comment}
\begin{table}[]
\begin{threeparttable}
\caption{AUC}
\footnotesize
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{model/graph type} & Scale-free & ER & Community
& Small-world \\ \midrule
{\ul \textbf{Iterative algorithm:}}  &             &                 &                 &                  \\
\hspace{0.1cm}  ADMM   &  0.9440 $\pm$ 0.0050  &   0.9435 $\pm$ 0.0062   &  0.9507 $\pm$ 0.0063  &  0.9852 $\pm$  0.0029               \\
\hspace{0.1cm} primal-dual splitting   & 0.9336 $\pm$  0.0072 & 0.9689 $\pm$ 0.0049 &  0.9038 $\pm$ 0.0056 &  0.9125 $\pm$ 0.0072  \\
{\ul \textbf{Learned to optimise:}}  &             &                 &                 &                  \\
\hspace{0.1cm}  GLAD \cite{Shrivastava2020GLAD}               & 1  $\pm$ 0  &    1  $\pm$ 0        &   1  $\pm$ 0   &    1  $\pm$ 0      \\
\hspace{0.1cm}  Deep-graph \cite{belilovsky17a}                &  0.5127 $\pm$ 0.0168  & 0.7411 $\pm$ 0.0319  & 0.5856 $\pm$ 0.0210 &   0.5293 $\pm$ 0.0098     \\
{\ul \textbf{Proposed:}}             &             &                 &                 &                  \\
\hspace{0.1cm} recurrent unrolling & 0.9637 $\pm$ 0.0052 &  0.9539 $\pm$ 0.0071    & 0.9234 $\pm$ 0.0073    & 0.9635 $\pm$ 0.0051  \\
\hspace{0.1cm}  unrolling                     & 0.9932 $\pm$ 0.0010   &  0.9913 $\pm$ 0.0014     & 0.9889 $\pm$ 0.0017    &   0.9838 $\pm$ 0.0049    \\
\hspace{0.1cm} L2G   & \bf{0.9991 $\pm$ 0.0003}           & \bf{0.9985 $\pm$ 0.0009}   & \bf{0.9929 $\pm$ 0.0009}  & \bf{0.9909 $\pm$ 0.0002}                  \\ \bottomrule
\end{tabular}
\end{threeparttable}
\end{table}

\end{comment}






\begin{comment}
\begin{algorithm}[h!]
\caption{Learning to learn graph topology (L2G)}
\label{alg:L2G}
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE Training sample batches $\{(\*z_i, \*w_i)\}_{i=1}^n$, evaluation sample batches $\{ \*z_i \}_{i=n+1}^N$, number of unrolls $T$.
 
 {\bf TRAIN} 
 \FOR {$i = 1, 2, \dots, n$}
 
 \STATE $\mathbf{w}_i^{(1)}, \mathbf{w}_i^{(2)}, \dots, \mathbf{w}_i^{(T)} \leftarrow \texttt{Unrolling}(\*z_i, T)$ from Algorithm \ref{alg:unrolling}

 \underscore{\textit{TopoDiffVAE Module:}}
 \STATE $\quad$ Let $G_x^{(i)}$ and $G_y^{(i)}$ be the binary structure of $\*w_i^{(T)}$ and $\*w_i$ extracted with threshold $\epsilon$.
 \STATE $\quad$  $\*h_x^{(i)} = \texttt{ENC}(G_x^{(i)})$ and $\*h_y^{(i)} = \texttt{ENC}(G_y^{(i)})$
 \STATE $\quad$ $\boldsymbol{\delta}^{(i)} = \*h_y^{(i)} - \*h_x^{(i)}$ and  $\*d^{(i)} \sim \mathcal{N}(\*0, \*I)$
 \STATE $\quad$ $\hat{\*w_i} = \texttt{DEC}()$
 
 \ENDFOR
 \STATE 
 \RETURN $\mathbf{w}^{(T)}$
\end{algorithmic} 
\end{algorithm}


\end{comment}


% unrolling solely can learn a graph. 
\begin{comment}
It is possible to learn a meaningful mapping form data to graph topology with the unrolling module solely by minimising the corresponding loss $\mathcal{L}_{\text{unroll}}$ such that
\begin{equation}
\label{eq: unrolling_loss}
    \min_{\theta_{\text{unroll}}} \  \mathcal{L}_{\text{unroll}} := \mathbb{E}_{\*w \sim \mathcal{G}} \Big[ \sum_{t=1}^{T} \tau^{T-t} \frac{||\*w^{(t)} - \*w||^2_2}{||\*w||^2_2} \Big]
\end{equation}%
 \par
\end{comment}




\Note{end2end? put into next subsection} The training procedure of TopoDiffVAE is integrated with that of unrolling module in an end-to-end fashion. The loss contribution of TopoDiffVAE is 
\begin{equation}
\label{eq: loss_vae}
    \mathcal{L}_{\text{TopoDiffVAE}} := \mathbb{E}_{\*w \sim \mathcal{G}} \Bigg[ || \hat{\*w}^{\text{(refine)}} - \*w||^2_2 + \beta_{\text{KL}} \mathcal{D}_{\text{KL}}\Big( q_{\phi}(\*z|G_X, G_Y) || \mathcal{N}(\*0, \*I) \Big) \Bigg] 
\end{equation}%


= Comments on the existing methods: 
  (1) estimating graph weights and structure (graph connectivity) together. 
  (2) structural prior are modelled explicitly as convex regularisers, e.g. sparsity, Laplacian constraints \cite{Kumar2019}, log barrier. Many sophisticated structures are largely ignored, e.g. scale-free.
  (3) Some regularisers are added to prevent trivial solutions, e.g. the log barrier to prevent isolated nodes, but conflicts with other structure, e.g. sparsity. 
  (4) Iterative takes long to converge.
  (5) Optimally tuning penalty parameters are not trivial. \par






\begin{table}[]
\caption{Structural Metrics}
\footnotesize
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{1}{c}{metric / model} & groundtruth & PDS                  & Deep-Graph \cite{belilovsky17a}           & unrolling            & L2G                  \\ \midrule
{\ul \textbf{BA:}}                 &    \multicolumn{1}{l}{}         & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\hspace{0.1cm} AUC      &    -         & 0.9336$\pm$.009      & 0.5127$\pm$.017      & 0.9932$\pm$.001      & 0.9991$\pm$.0003    \\
\hspace{0.1cm} PowerLawGOF                        &             &                      &                      &                      &                      \\
{\ul \textbf{SBM:}}                &    \multicolumn{1}{l}{}         & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\hspace{0.1cm} AUC     &  -  &  0.9256 (0.0062)   &   0.5856 (0.0210)   &    0.9889 (0.0017)      &  0.9929 (0.0019)  \\
\hspace{0.1cm} community score   & 0.4633 (0.0022)  &     0.4808 (0.0024)   &    0.3438 (0.0060)   &     0.4581 (0.0011)    & 0.4691 (0.0027)          \\
  {\ul \textbf{WS:}} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
 \hspace{0.1cm} AUC &  -    &   0.9125 (0.0072)    &  0.5293 (0.0098)     &  0.9838 (0.0049)     &   0.9909 (0.0002)  \\
\hspace{0.1cm} average shortest path  &   2.3339 (0.0277)    &    2.6558 (0.2037)     &    1.1363 (0.0083)   &   2.3278 (0.0398)  &           2.3306 (0.0414)  \\
\hspace{0.1cm} clustering coefficient     & 0.3228 (0.0182)  &   0.5147 (0.0352)      &    0.9060 (0.0040)    &    0.4331 (0.0164)   &       0.3818 (0.0142) \\ \bottomrule
\end{tabular}
\end{table}







\begin{table}[]
\label{table:gmse}
\begin{threeparttable}
\caption{GMSE}
\footnotesize
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{model/graph type} & Scale-free & ER & Community
& Small-world \\ \midrule
{\ul \textbf{Iterative algorithm:}}  &             &                 &                 &                  \\
\hspace{0.1cm}  ADMM   &  0.4094 $\pm$ 0.0120  &   0.3547 $\pm$ 0.0120   &  0.3168 $\pm$ 0.0226  &  0.2214 $\pm$  0.0151               \\
\hspace{0.1cm} PDS   & 0.4033 $\pm$  0.0072 & 0.3799 $\pm$ 0.0085  &  0.3111 $\pm$ 0.0147 &  0.2180 $\pm$ 0.0117    \\
{\ul \textbf{Learned to optimise:}}  &             &                 &                 &                  \\
\hspace{0.1cm}  GLAD \cite{Shrivastava2020GLAD}               &  1.1230 $\pm$ 0.1756   &   1.1365 $\pm$ 0.1549              &   1.4231 $\pm$ 0.2625    &  0.9999 $\pm$ 0.0001         \\
\hspace{0.1cm}  Deep-graph$^\ast$ \cite{belilovsky17a}                &  0.8423 $\pm$ 0.0026 & 0.8179 $\pm$ 0.0269  & 0.8931 $\pm$ 0.0103 &  0.8498 $\pm$ 0.0017     \\
{\ul \textbf{Proposed:}}             &             &                 &                 &                  \\
\hspace{0.1cm} recurrent unrolling & 0.3018 $\pm$ 0.0080 &  0.2885 $\pm$ 0.0075    & 0.2658 $\pm$ 0.0108  & 0.2007 $\pm$ 0.0081  \\
\hspace{0.1cm}  unrolling                     & 0.1079 $\pm$ 0.0047   &  0.0898 $\pm$ 0.0067     & 0.1199 $\pm$ 0.0064     &   0.1028 $\pm$ 0.0073    \\
\hspace{0.1cm} L2G   & \bf{0.0594 $\pm$ 0.0044}           & \bf{0.0746 $\pm$ 0.0042}   & \bf{0.0735 $\pm$ 0.0051}  & \bf{0.0513 $\pm$ 0.0060}                  \\ \bottomrule
\end{tabular}
\begin{tablenotes}
  \footnotesize
  \item $^\ast$ GMSE may not favour Deep-graph as it learns binary structures only. We also report AUC in Table[].
\end{tablenotes}
\end{threeparttable}
\end{table}

\begin{table}[]
\caption{Structural Metrics}
\footnotesize
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{1}{c}{metric / model} & groundtruth & PDS                  & Deep-Graph \cite{belilovsky17a}           & unrolling            & L2G                  \\ \midrule
{\ul \textbf{BA:}}                 &    \multicolumn{1}{l}{}         & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\hspace{0.1cm} AUC      &    -         & 0.934$\pm$.009      & 0.5127$\pm$.017      & 0.993$\pm$.001      & 0.9991$\pm$.0003    \\
\hspace{0.1cm} PowerLawGOF                        &             &                      &                      &                      &                      \\
{\ul \textbf{SBM:}}                &    \multicolumn{1}{l}{}         & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\hspace{0.1cm} AUC     &  -  &  0.9256 (0.0062)   &   0.5856 (0.0210)   &    0.9889 (0.0017)      &  0.9929 (0.0019)  \\
\hspace{0.1cm} community score   & 0.4633 (0.0022)  &     0.4808 (0.0024)   &    0.3438 (0.0060)   &     0.4581 (0.0011)    & 0.4691 (0.0027)          \\
  {\ul \textbf{WS:}} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
 \hspace{0.1cm} AUC &  -    &   0.9125 (0.0072)    &  0.5293 (0.0098)     &  0.9838 (0.0049)     &   0.9909 (0.0002)  \\
\hspace{0.1cm} average shortest path  &   2.3339 (0.0277)    &    2.6558 (0.2037)     &    1.1363 (0.0083)   &   2.3278 (0.0398)  &           2.3306 (0.0414)  \\
\hspace{0.1cm} clustering coefficient     & 0.3228 (0.0182)  &   0.5147 (0.0352)      &    0.9060 (0.0040)    &    0.4331 (0.0164)   &       0.3818 (0.0142) \\ \bottomrule
\end{tabular}
\end{table}




\begin{wrapfigure}{R}{0.55\textwidth}
\vspace{-10pt}
\centering
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width = 1\linewidth]{Fig/GLAD_perturbation_AUC.png}
    \subcaption{AUC}
    \label{fig:exp_noisy_SBM_APS}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width = 1\linewidth]{Fig/GLAD_perturbation_GMSE.png}
    \subcaption{GMSE}
    \label{fig:exp_noisy_ER_APS}
\end{subfigure}%
\caption{Sensitivity to perturbations for positive definiteness}
\label{fig: syn_exp_GLAD}
\end{wrapfigure}





\begin{comment}
The backward steps are proximal mappings of non-differentiable regularisations $\Omega_1(\*w) = \mathcal{I}_{\{\*w \geq 0\}}(\*w)$ and $\Omega_2(\mathcal{D}\*w) = - \alpha \mathbf{1}^{\top}\log(\mathcal{D}\*w)$. Specifically,
\begin{equation}
    \text{prox}_{\gamma^{(t)}, \Omega_1}(\*w) = \min\{\*0, \*w\}
\end{equation}%
\begin{equation}
   \text{prox}_{\gamma^{(t)}, \Omega_2}(\*v)_i = \frac{v_i - \sqrt{v_i^2 + 4\alpha^{(t)} \gamma^{(t)}}}{2}
\end{equation}

from the model-based graph learning, which unfold the iterative procedure that solves the objective \cite{Kalofolias2016}
\Note{SC: need transition}
\begin{equation}
\label{eq: graph_leanring_objective_with_log}
    \min_{\*w} \ 2\*w^{\top}\*y + \mathcal{I}_{\{\*w \geq 0\}}(
    \*w) - \alpha \mathbf{1}^{\top}\log(\mathcal{D}\*w) + \beta||\*w||^2_2
\end{equation}%
where the log-barrier on node strength $\mathcal{D}\*w$ is to prevent isolated nodes and the $l_2$ norm on edge weights force the estimation to be smooth. $\alpha$ and $\beta$ are corresponding penalty hyper-parameters.
% why not lasso:
It should be note that the popular lasso term on edge weights to encourage sparsity is implicitly encoded in the first two terms such that given $\*w \geq 0$, $2\*w^{\top}\*y = 2\*w^{\top}(\*y-\sfrac{\lambda}{2}) + \lambda||\*w||_1$. Also, the unrolling module is made to be flexible 
%with primal-dual splitting iterative algorithm 
that allows arbitrary convex regularisers on edge weights or node strength. 
%We simply choose the most popular log-barrier and $l_2$ in literature.
To some extent, these regularisers have implications on the structural properties of learned graph, but possibly less expressive to sophisticated structures e.g. scale-free, small-world and community-like networks, which motivates TopoDiffVAE in Section~\ref{sec: method_TopoDiffVAE}. \par
\end{comment}





%The mapping is one-to-one as 
%Note that $\mathcal{P}$ is surjective as the node ordering is fixed. 
%where $\*w_X$ and $\*w_Y$ are the input and output half-vectorized graph representation, respectively, and the latent code $\*z$ is drawn from a prior distribution $P(\*z)$.
% many interesting topological properties are difficult to  are difficult to be expressed with a compact mathematical expression.
%Different from \cite{jin2020-graph2graph}, the mapping is not multimodal in our case as the unrolling module returns permutation-invariant estimation. \par
%Notice that the mapping from $\mathcal{X}$ to $\mathcal{Y}$ is surjective as the node ordering is fixed. The goal of {\bf TopoDiffVAE} is not to generate a new graph topology; rather it refines the estimation obtained from the unrolling module by improving the topological properties encoded in its groundtruth graph. To this end, we assume the marginal probability $P(G_Y)$ is adequately expressive to one class of graph topology. The learning processes should be separate for different graph topologies, e.g. for scale-free and small-world graphs.

%Notice that the mapping from $\mathcal{X}$ to $\mathcal{Y}$ is surjective as the node ordering is fixed. The goal of {\bf TopoDiffVAE} is not to generate a new graph topology; rather it refines the estimation obtained from the unrolling module by improving the topological properties encoded in its groundtruth graph. To this end, we assume the marginal probability $P(G_Y)$ is adequately expressive to one class of graph topology. The learning processes should be separate for different graph topologies, e.g. for scale-free and small-world graphs.

%The main motivation behind the TopoDiffVAE module s to enable the proposed model to better adapts to the implicit topological properties present in the training graphs. To this end, in the forward propagation, TopoDiffVAE takes the gradient descent estimate $\*r_1^{(t)}$ as input and extract a binary graph structure $G_X$ 
% We first extract the binary edge structure $G_X$ of $\*r_1^{(t)}$ by setting the edge weights less than $\eta$ to zero and those above $\eta$ to one. We are thus given the training pairs $\{(G_X, G_Y)\}$ drawn from their joint distribution $P(G_X, G_Y)$, where $G_Y \in \mathcal{G}$ is the binary graph structure that corresponds to the groundtruth graph representation $\*w$. 


%recovering graphs with different structures, e.g. sparse, scale-free, small-world, component graphs with synthetic groundtruth. A big improvement on accuracy and speed of convergence is witnessed in experiments. We also transfer the pre-trained models to learn an insightful graph that reveals the relationship between S\&P 100 stocks and brain functional connectivity of Autism, which shows the proposed methods can be applied to real-world scenarios. \par

